Prediction Accuracy of Learning in Games : Follow-the-Regularized-Leader meets Heisenberg

We investigate the accuracy of prediction in deterministic learning dynamics of zero-sum games with random initializations, specifically focusing on observer uncertainty and its relationship to the evolution of covariances. Zero-sum games are a prominent field of interest in machine learning due to their various applications. Concurrently, the accuracy of prediction in dynamical systems from mechanics has long been a classic subject of investigation since the discovery of the Heisenberg Uncertainty Principle. This principle employs covariance and standard deviation of particle states to measure prediction accuracy. In this study, we bring these two approaches together to analyze the Follow-the-Regularized-Leader (FTRL) algorithm in two-player zero-sum games. We provide growth rates of covariance information for continuous-time FTRL, as well as its two canonical discretization methods (Euler and Symplectic). A Heisenberg-type inequality is established for FTRL. Our analysis and experiments also show that employing Symplectic discretization enhances the accuracy of prediction in learning dynamics.

==> Introduction.tex <==
\section{Introduction}

% Here is a problem.
% It is an interesting problem.
% It is an unsolved problem.
% Here is my approach.
% My approach works.

%Motivation:

%\begin{itemize}

%\item Differential entropy is constant in alternating MWU and alternating GDA. However, the observer uncertainty evolution (i.e., expanding or stay bounded) in alternating updates is captured by covariance.

%\item Review of ICML submission :
%\textbf{Question} : It was unclear from the paper what additional insights one can hope to obtain by studying the game evolution from a covariance perspective.
%\textbf{Answer} : The analysis of game theoretic dynamics from a co-variance perspective provides practically valuable insights which are totally missing in the standard analysis of trajectories (i.e. tracking of the mean of the distribution). We provide three such perspectives below:

%1) Quantifying the numerical stability of orbits.\\
%E.g. in practice due to discretization errors when an update is performed on a learning dynamic there is some inherent randomness of the mapping due to small computation errors. So it is actually a rather useful practical perspective of thinking our dynamics initialized not just with a single point but with a distribution and then study not only how the mean evolves over time, but also how and whether the uncertainty/errors spread. For example the exponential increases of the variances in the case of Euler schemes clearly implies that such infinitesimal errors cannot be ignored even for a relatively small time horizon in constrast the symplectic schemes which show much better stability.

%2) A second perspective is about using these estimates as a tool for explainable AI in multi-agent systems.\\
%E.g. in many recent AI systems such as GANs are designed around zero-sum games. In such systems, it would be very beneficial if a system did not just provide a single prediction/outcome but simultaneously provided some estimate about how confident it was in these predictions. In such systems the mean would provide the answer but the covariance matrix would encode the uncertainty. Thus understanding not only the evolution of the means but of the co-variance matrix becomes a very useful tool and even a way to distinguish between learning dynamics with similar regret guarantees. For example between two algs with similar regret guarantees (in expectation) we would prefer the algorithm that minimizes the spread of uncertainty.

%3) A third perspective is that of information theory and capturing ambiguity in decision making.\\ 
%One can think of the probability distribution played by an agent as their beliefs about which is the best action for them. E.g. the first action is choosing to go to university A whereas the second action is going to university B. So now if we only report a single probability distribution (e.g. $50\% 50\%$) it does not allow us to encode the uncertainty or ambiguity of the agent. Think for example three different cases:
 %In the first case the agent knows that the school are identically desirable for them, then the appropriate way to encode this is with a single Dirac distribution at $50\% 50\%$.
 %In the second case the agent knows absolutely nothing about schools A, B. Then the correct way to encode this is a uniform measure on the $[0,1]$ interval.
 %In the third case contingent on the outcome of whether the student gets scholarship or not (let's say this happens with $50\%$ chance), their prefer school A, otherwise school B. In all three cases the mean of the distribution is at $50/50$ but they define totally different behavioral/information theoretic settings. Here is where access to covariance information becomes critical as it affects the future trajectory of the system and allows us to capture how its affects both the mean belief as well as the co-variances/uncertainty of the agents over time.
 
%\end{itemize}



%\section{Introduction}
In recent years understanding the behavior of learning algorithms in repeated games has attracted increasing interests from the machine learning community~\citep{lanctot2017unified,yang2020overview}. Follow-the-Regularized-Leader (FTRL) algorithm~\citep{abernethy2009competing,shalev2012online}, arguably the most well known class of no-regret dynamics, plays a prominent role in analysis of behavior of learning algorithms. The behavior of such online learning algorithm in zero-sum games has been a particularly intense object of study as zero-sum games related to numerous recent applications and advances in AI such as, achieving super-human performance in Go~\citep{silver2016mastering}, Poker~\citep{brown2018superhuman} and Generative Adversarial Networks (GANs)~\citep{goodfellow2014generative} to name a few.
%, and multi-agent learning for AI systems \citep{balduzzi2020smooth,leibo2019autocurricula}. 

Predicting players' long term behaviors in a repeated game is a fundamental and challenging problem \citep{nachbar1997prediction,cesa2006prediction}. The conventional wisdom in this regard is that players' strategies will eventually converge to some equilibrium.
However, recent studies have shown that such a belief usually fails  for several learning dynamics \citep{nagarajan2020chaos,milionis2023impossibility}. In particular, FTRL dynamics do not even converge in zero-sum games and exhibit complex behaviors such as Poincaré recurrence and even chaos \citep{MPP18,cheung2021chaos}. 

%This makes predicting their behavior and outcome of the learning algorithms difficult as an infinitesimal small perturbation of the initial conditions may be very quickly amplified by the learning algorithms. 

% {Yi:} Predicting players' long term behaviors in a repeated game is a fundamental and challenging problem \citep{nachbar1997prediction,cesa2006prediction}. The conventional wisdom in this regard is that players' strategies will eventually converge to some equilibrium. However, recent studies have shown that such a belief usually fails  for several learning dynamics \citep{nagarajan2020chaos,milionis2023impossibility}. In particular, FTRL dynamics do not even converge in zero-sum games and exhibit complex behaviors such as recurrence and divergence \citep{MPP18,BP18}. This line of research model the learning algorithm as a determinstic dynamical system, and thus the following equality holds :
%\begin{align*}
%  \text{Input : accurate current strategies  Accurate future strategies.}
%\end{align*}
%However, in partical, an observer may have some uncertainty about the current strategy used by players. This kind of uncertainty is common both from a game-theoretic perspective (i.e., the unknown external action on agents’ preference) as well as from a Machine Learning perspective (i.e., noise introduced in the training process). Thus for such an observer, he will ask :
%\begin{align*}
%  \text{Slightly inaccurate current strategies + Learning algorithms = Exact future strategies.}
%\end{align*}



Chaos in learning dynamics indicates that the main obstacle in predicting long term behavior is its sensitive dependence on initial conditions, i.e., small perturbation of initial condition will end up with dramatically different outcomes. Figure \ref{Tra 3d} illustrates that in a repeated Rock-Paper-Scissor game, the evolution of many orbits starting from a small region when both players use Alternating Multiplicative Weights Update. Figure \ref{Tra 3d} shows that even small initial noise can be amplified and make the accurate prediction difficult. Motivated by this example, we naturally formulate the following question:

\textit{How to track the accuracy of prediction in learning dynamics?}

%In addition to these intrinsic complexities of the learning dynamics, another obstacle that prevents an observer from accurately predicting players' future behaviors is the uncertainty about the initial strategies of players. This kind of uncertainty is common both from a game-theoretic perspective (i.e., the unknown external action on agents’ preference) as well as from a Machine Learning perspective (i.e., noise introduced in the training process). 
%Imagine an observer who is observing two players playing a game and is aware of the learning algorithms used by players, but has a slight uncertainty described by a distribution about their current strategies, and we would like to know :

%\textit{What level of accuracy can the observer achieve in predicting future behaviors of players?}

\begin{figure*}[t]
\centering
\subfigure[t = 0]{
\includegraphics[clip,width=0.65\columnwidth]{AltMWU_t0.png}
}
\subfigure[t = 50]{
\includegraphics[clip,width=0.65\columnwidth]{AltMWU_t50.png}
}
\subfigure[t = 80]{
\includegraphics[clip,width=0.65\columnwidth]{AltMWU_t80.png}
}
\subfigure[t = 130]{
\includegraphics[clip,width=0.65\columnwidth]{AltMWU_t130.png}
}
\subfigure[t = 150]{
\includegraphics[clip,width=0.65\columnwidth]{AltMWU_t150.png}
}
\subfigure[t = 200]{
\includegraphics[clip,width=0.65\columnwidth]{AltMWU_t200.png}
}
\caption{Evolution of 400 initial conditions (blue points) for one player using (\ref{2pMWUA}) in Rock-Paper-Scissors game, the red point is the expectation of initial samples. At time $t=0$, these point are uniformly sampled in a small square with a side length of 0.05 on the simplex. At time $t=50, 80, 130$, the shape of square has been destroyed. At time $t=150,200$, it appears that these points have no relation to each others and are randomly located on the simplex. 
%If an observer at $t=0$ only knows that an initial condition lies within the small square, he will have significant uncertainty about the location of this initial condition at time $t=200$. 
Moreover, the evolution of expectation (red point) cannot accurately predict future outcomes, as sample points in subsequent times may deviate significantly from the expected value.}
\label{Tra 3d}
\end{figure*}




At first glance, since learning algorithms such as FTRL are completely deterministic, accurate predictions for players' future behaviors can be made by methods such as tracking the expectation of the distribution on strategy at every time node (assuming that he can access the distribution), if the observer's uncertainty is initially small, for example, if he knows that the players' actual strategy lies within a narrow region. Surprisingly, this belief is incorrect. One remarkable aspect of several learning dynamics, like Multiplicative Weights Updates (FTRL with negative entropy regularizer), is that slight initial deviation can give rise to significantly divergent strategy trajectories for players over extended periods \citep{sato2002chaos,galla2013complex}. The phenomenon is exemplified in Figure \ref{Tra 3d} to provide an explanation. As depicted, the observer's uncertainty is initially low (the real mixed strategy lies within a small blue square on the simplex). However, over time, these points can become widely dispersed and appear randomly distributed on the simplex. Moreover, tracking the expectation (red point) fails to accurately prediction as a large portion of  points  will deviate significantly from the expectation; in terms of statistics, the \textbf{(co)variance} of the distribution can be large over time, hindering accurate predictions of players' future behaviors.
%Consequently, the learning dynamics can significantly amplify small deviations from expectations in the initial time, resulting in prediction failure. 
%Recently, the machine learning community has also focused on various formal qualitative characteristics of this phenomenon, such as Lyapunov chaos \citep{cheung2019vortices,CP2020}.

Given the significance of predicting learning outcomes in games and the aforementioned challenges, it is crucial to understand the evolution of variance about observer's uncertainty distribution through the the learning dynamics. The most relevant paper in this direction is \citep{CPT2022}, which utilized \textit{differential entropy} instead of variance as their metric of uncertainty. Differential entropy serves as an analogue of standard Shannon entropy for continuous variables and demonstrates that it grows linearly fast in two-player zero-sum games, quantifying the amount of excess information an outsider must gather to keep track of the uncertain system evolution. However, as we will show in following, differential entropy cannot capture the uncertainty evolution of the \emph{alternating} update rule of game dynamics. 

In this work, after highlighting some drawbacks of differential entropy, we will study the evolution of covariance matrix through the lens of the Hamiltonian formulation of FTRL \citep{PB1,wibisono2022alternating}. Specifically,  given a random system initialization (in the relevant system state-space), we will focus on the evolution of variances of the related random variables in two popular updating rules: simultaneous update and alternating update. This perspective studies the evolution of covariance closely related to the well known \emph{Heisenberg Uncertainty Principle} in quantum mechanics, which states that one cannot measure the momentum and position of a microscopic particle accurately at the same time, i.e., $\Delta p\Delta q\ge h$.  The Hamiltonian formulation of FTRL endows the cumulative strategy and payoff of each agent the roles of position $q$ and momentum $p$ of each particle. Once the initialization is randomized, the deterministic learning dynamics still makes the cumulative strategy and payoff random variables whose mean and covariance matrix is related to that of the initialization. Therefore, it is natural to ask how the variances of cumulative strategies and payoffs evolve with FTRL dynamics. As what is implied from Heisenberg Uncertainty, information on standard deviations (variances, covariance matrices) measures the \emph{accuracy of prediction} in learning dynamics. 


\paragraph{Our contributions.}We highlight our main contributions as following:
%\paragraph{Our contributions.}
%In this paper we study differential entropy and covariances in FTRL for two-player zero-sum games. We investigate the evolution of observer uncertainty measured by these two quantities in two popular updating rules: simultaneous update and alternating update. We establish the following results as main contributions, which also serve as our answers to the three problems we previously proposed : 
\begin{itemize}[leftmargin=*]
\item We prove differential entropy remains constant when two players alternatively update their strategies. Therefore, it is not a strong notation for capturing the evolution of uncertainty in alternating update, see Proposition \ref{entropya};
\item We propose the covariance matrix as an uncertainty measurement which captures both simultaneous and alternating updates, with rate of increasing calculated concretely in Euclidean regularized FTRL, see Theorem \ref{Covariance Evolution in FTRL with Euclidean Regularizer}. Our results imply a separation between simultaneous and alternating plays : the covariance of alternating plays has a quadratic growth rate that match the continuous time dynamics, while simultaneous plays have an exponential growth rate;
\item For FTRL with general regularizers, a Heisenberg type inequality on variances of cumulative strategy and payoff is obtained, i.e., $\Delta X_{i,\alpha}\Delta y_{i,\alpha}\ge\text{positive constant}$. This inequality indicates a general uncertainty principle, tradeoff between accuracy in strategy spaces versus payoff spaces for game dynamics, see Theorem \ref{prop:nonlinear}. The inequality also imposes an interesting constrains on the  predictive ability of an observer, which can be summarized as 
    \textit{an observer cannot accurately predict the actual strategies of two players at the same time when they use alternating update rule} 
see Corollary \ref{UIs}. In Figure \ref{UI} we present an example to illustrate this point. 
\end{itemize}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{Uncertainty_ineq.png}
    \caption{The two curves represent the evolution of sample variances for the strategies on 300 random samples of two players when they use (\ref{2pMWUA}). The appearance time of local \textbf{minima} on the blue curve usually coincides with the local \textbf{maxima} on the red curve or very close to them, and vice versa. This implies that the variance of strategies of the two players cannot be small at the same time.}
    \label{UI}
\end{figure}

%This perspective is closely related to the well known as \emph{Heisenberg Uncertainty Principle} in quantum mechanics, which captures that one cannot measure the momentum and position of a microscopic particle accurately at the same time, i.e., $\Delta p\Delta q\ge h$.  The Hamiltonian formulation of FTRL endows the cumulative strategy and payoff of each agent the roles of position $q$ and momentum $p$ of each particle. Once the initialization is randomized, the deterministic learning dynamics still makes the cumulative strategy and payoff random variables whose mean and covariance matrix is related to that of the initialization. Therefore, it is natural to ask how the variances of cumulative strategies and payoffs evolve with FTRL dynamics. As what is implied from Heisenberg Uncertainty, information on standard deviations (variances, covariance matrices) measures the \emph{accuracy of prediction} in learning dynamics.  %To our best knowledge, understanding the predicability of learning dynamics through the evolution of variances is missing in literature, even for gradient descent ascent algorithm.


%recently introduced a framework to study the evolution of uncertainty of (\ref{2pMWUS}) in zero-sum games and variants thereof. The key idea is to model the uncertainty as a probability distribution over a set of possible initial conditions. Given this formulation they 

%\begin{itemize}
%\item Which metric of uncertainty quantitatively describes "risk" and "deviation from expectation" alongside the learning dynamics?
%    \item \textit{Which metric of uncertainty is suitable for measuring the evolution of uncertainties alongside the learning dynamics?}
%    \item \textit{Could subtle differences in implementation of  learning dynamics result to significant differential in their performance from an uncertainty perspective?}
%    \item \textit{Can we identify some constraints that limit the predictive ability of an observer who possesses inherent information about the game process, such as the payoff functions and algorithms used by the players?}
%\end{itemize}


%In this work, we also model the uncertainty as a distribution defined on players' initial conditions, following \citep{CPT2022}. After highlighting some drawbacks of differential entropy, we will be introducing a novel perspective in quantifying uncertainty, motivated by the Hamiltonian formulation of FTRL \citep{PB1,wibisono2022alternating} and the uncertainty principle from quantum mechanics. Specifically,  given a random system initialization (in the relevant system state-space) we will be focusing on the evolution of \textit{variances} of the related random variables. This perspective is closely related to the well known as \emph{Heisenberg Uncertainty Principle} in quantum mechanics, which captures that one cannot measure the momentum and position of a microscopic particle accurately at the same time, i.e., $\Delta p\Delta q\ge h$.  The Hamiltonian formulation of FTRL endows the cumulative strategy and payoff of each agent the roles of position $q$ and momentum $p$ of each particle. Once the initialization is randomized, the deterministic learning dynamics still makes the cumulative strategy and payoff random variables whose mean and covariance matrix is related to that of the initialization. Therefore, it is natural to ask how the variances of cumulative strategies and payoffs evolve with FTRL dynamics. As what is implied from Heisenberg Uncertainty, information on standard deviations (variances, covariance matrices) measures the \emph{accuracy of prediction} in learning dynamics.  %To our best knowledge, understanding the predicability of learning dynamics through the evolution of variances is missing in literature, even for gradient descent ascent algorithm.

%\textcolor{red}{To add Our results and techniques section here.}
\input{results_techniques}


\begin{comment}
\textbf{Results and contributions.} In this paper, we focus on the FTRL with Euclidean norm regularizer, which is arguably the most fundamental case of FTRL algorithm. As a template to study the evolution of variances of cumulative strategies and payoffs, we investigate three variants of FTRL which are commonly used in theoretical analysis and application, i.e., continuous time, Euler discretization, and symplectic discretization of FTRL. Throughout this paper, we denote $X_i(t)$ and $y_i(t)$ the cumulative strategy and payoff vectors of player $i$. The main result can be stated in the perspective of player-1 as follows,
\begin{theorem}[Informal]
Let $A=A^{(12)}$ be the payoff matrix of the first player in a two-player zero-sum game. Suppose FTRL with Euclidean norm regularizer is used to update their strategies, and at some point $t_0>0$, randomness is introduced such that $X_1(t_0)$ and $y_1(t_0)$ are random vectors with $P(t_0)$ the covariance matrix of $(X_1(t_0),y_1(t_0))$. Then the following statements holds:
\begin{enumerate}
\item Continuous time FTRL: if $AA^{\top}$ is non-singular, variances of $X_1(t)$ and $y_1(t)$ are bounded for all $t>t_0$; if $AA^{\top}$ is singular, variances of $X_1(t)$ increase at order $\Theta(t^2)$ and $y_1(t)$ stay bounded.
\item Euler method: variances of $X_1(t)$ and $y_1(t)$ increase exponentially for all $t>t_0$;
\item Symplectic Euler method: if $AA^{\top}$ is non-singular, variances of $X_1(t)$ and $y_1(t)$ are bounded for all $t>t_0$; if $AA^{\top}$ is singular, variances of $X_1(t)$ increase at order $\Theta(t^2)$, $y_1(t)$ stay bounded.
\end{enumerate}
\end{theorem}

Note that conditions on $AA^{\top}$ can be satisfied by different games in real life, e.g., the payoff matrix of the Rock-Paper-Scissors game makes $AA^{\top}$ singular, but that of meta-payoff matrix of AlphaStar is non-singular\citep{czarnecki2020real}. Especially, if $A$ is not square, then there must be one player whose $AA^{\top}$ is singular.
%Precisely, by ``generically" we mean that for almost all payoff matrices $A$, the square matrix $AA^{\top}$ has no zero eigenvalues since the set of matrices such that $AA^{\top}$ have zero eigenvalues is of measure zero. Furthermore, we show that if $AA^{\top}$ has zero eigenvalues, then Simultaneous GDA exponentially increases the variances of cumulative strategies and payoffs, while the Symplectic GDA increases the variances of cumulative strategies at order $\Theta(t^2)$ and keeps the variances of cumulative payoff bounded.

Differential entropy of continuous random variables is a central concept in information theory, and it is a canonical way of measuring uncertainty a system. The differential entropy is closely related to the covariance matrix of random vectors through the following inequality (Theorem 8.6.5, \citep{thomas2006elements}):
\begin{equation}\label{entropy-covariance}
h(X)\le\frac{1}{2}\log\left((2\pi e)^n\det(P)\right)
\end{equation}
where $X$ is a random vector in $\mathbb{R}^n$ and $P$ is the covariance matrix of $X$. Uncertainty analysis in learning dynamics based on differential entropy was proposed in \citep{CPT2022}, where the linear growth of differential entropy with multiplicative weights update is established, which conjecturally yields a lower bound for the growth of covariances based on \eqref{entropy-covariance}. This leaves the specific growth rate of covariance with MWU and GDA unaddressed. In the current paper, we provide an exact growth rate of covariances in different discretization settings of Euclidean norm regularized FTRL. Whether the techniques of covariance and differential entropy can be bridged so that we can have a complete understanding on quantifying uncertainty evolution in general learning algorithms is an important direction for future research.

%The case that the payoff matrix is not full-rank is also quantified in our analysis, saying that the Simultaneous GDA exponentially increases the variances of cumulative strategies and payoffs, while the Symplectic GDA increases the variances of cumulative strategies at order $\mathcal{O}(t^2)$ and keeps the variances of cumulative payoff bounded. 

%\paragraph{Connection to information theory.} \emph{Differential entropy} of continuous random variables, introduced by Claude Shannon, is a central concept in information theory, and is widely used in measuring uncertainty of a evolution system with randomness. The differential entropy is closely related to the covariance matrix of random vectors through the following inequality (Theorem 8.6.5, \citep{thomas2006elements}):
%\begin{equation}\label{entropy-covariance}
%h(X)\le\frac{1}{2}\log\left((2\pi e)^n\det(P)\right)
%\end{equation}
%where $X$ is a random vector in $\mathbb{R}^n$ and $P$ is the covariance matrix of $X$. For the case of multiplicative weights update (MWU) and its optimistic variant, the evolution of differential entropy is studied in \citep{CPT2022}, where the linear growth of differential entropy with MWU is established. Roughly speaking, one can conjecture based on \eqref{entropy-covariance} that the evolution of variances is at least of linear growth. Orthogonal to differential entropy with MWU, we provide an exponential increasing rate of variances of Gradient Descent Ascent (FTRL with Euclidean regularizer), and moreover, we propose that the evolution of variances with symplectic discretization (Alternating GDA) agrees with continuous time GDA, especially, both Alternating GDA and continuous time GDA keep the variances of cumulative payoff bounded.

\textbf{Limitations.} There are two major limitations of our techniques. Firstly, the covariance analysis heavily depends on a purely algebraic treatment of exponential map of matrix, which only works for linear Hamiltonian systems. For other regularizers of FTRL such as entropy regularizer, the Hamiltonian system is not linear, and there needs to be a nontrivial extension of current techniques before we can argue about the covariance evolution. Secondly, the step-size shows some subtlety of symplectic discretization. It is necessary to have equal step-size for both players so that the discretization is symplectic. Otherwise, our arguments cannot be trivially translated into that when players use different step-sizes. %These limitations yield promising directions of future research.
\end{comment}

%\textbf{Further related works.} 
%The family of FTRL algorithms in the continuous time and several their properties are investigated in \citep{MPP18}. However, it turns out the behaviors of discrete time algorithms is quite different from their continuous time counterpart. In the case of simultaneous gradient descent ascent with constant step size, the strategy orbits will not converge and keep away form its stationary points with an exponential rate \citep{mescheder2018training, gidel2018variational} and in the case of simultaneous multiplicative weights updates, the volumes of strategy orbits have fast growth rate and converge to the boundary of constrains \citep{bailey2018multiplicative, cheung2018multiplicative, CP2020}.  Alternating gradient-descent-ascent and its several variants are studied in \citep{gidel2018variational, bailey2020finite, zhang2019convergence, yang2020global}  and \citep{wibisono2022alternating} consider more general alternating mirror descent algorithms in constrained case.% In general, the dynamical behaviors of  algorithms in alternating setting are more similar to their continuous time partners, and usually they have faster convergence rate of regrets and other finer properties comparing to algorithms in simultaneous setting. 
% There are several other forms of uncertainties in game theory and min-max optimization. Another kind of uncertainty comes from the stochastic algorithms \citep{chavdarova2019reducing, luo2020stochastic, yang2020global}, where reducing the variance introduced by the algorithms is a main focus. Our results are orthogonal to aforementioned ones. %which consider the evolution of a random distribution on initial conditions that evolve according to some determined process. 
















